Life, the Metaverse and Everything: An Overview of Privacy, Ethics, and Governance in Metaverse

The metaverse is expected to be the next major evolution phase of the internet. The metaverse will have an impact on human society, production, and life. In this work, we analyze the current trends and challenges that building such a virtual environment will face. We focus on three major pillars to guide the development of the metaverse: privacy, governance, and ethical design, to guide the development of the metaverse. Finally, we propose a preliminary modular-based framework for an ethical design of the metaverse.

==> sections/modular_meta.tex <==
% Modular metaverse
Human-Centered Design (HCD) is a philosophy developed by Don Norman (among others)~\cite{norman2005human}. We consider this design approach for the metaverse as it requires the active involvement of users in the design process and decision-making.



\bparagraph{Human rights.} The metaverse should be accessible, diverse, and inclusive where every individual is welcome. Privacy is an intrinsic right of users, which they can protect using the available tools (PETs, avatar cretion). All the module are interchangeable and will use the current technologies such as Blockchain and DAOs to manage any decision taken in the metaverse (e.g., change in current policies about misbehaviour of users). All the active parts of the metaverse (including code) should be transparent and understandable to any member of the platform. This can reduce the complexity while voting (using DAOs) in the decision-making processes.

\bparagraph{Human effort.} The metaverse will include a reputation-based system that will be inherently attached to users and will be manage by Blockchain and DAOs. This reputation system will allow users to report misbehave and malpractice of malicious users while voting using DAOs. 


\bparagraph{Human Experience.} The metaverse will be an immmersive experience that will enable new ways of social interaction, content creation beyond our current real-world boundaries (e.g., regulations, geographical location, accessibility).



\begin{figure}
    \centering
    \includegraphics[width=.9\linewidth]{figures/solution/metaverse_ethical.pdf}
    \caption{Modular-based metaverse architecture motivated the 'Ethical Hierarchy of Needs' (licensed under CC BY 4.0). Each module is interchangeable according to the situation (e..g, current policies).} 
    \label{fig:modular:metaverse}
\end{figure}
